Time-dependent friction effects on vibrational infrared frequencies and line shapes of liquid water

From ab initio simulations of liquid water, the time-dependent friction functions and time-averaged non-linear effective bond potentials for the OH stretch and HOH bend vibrations are extracted. The obtained friction exhibits adiabatic contributions at and below the vibrational time scales, but also much slower non-adiabatic contributions, reflecting homogeneous and inhomogeneous line broadening mechanisms, respectively. Compared to the gas phase, hydration softens both stretch and bend potentials, which by itself would lead to a red-shift of the corresponding vibrational bands. In contrast, non-adiabatic friction contributions cause a spectral blue shift. For the stretch mode, the potential effect dominates and thus a significant red shift when going from gas to the liquid phase results. For the bend mode, potential and non-adiabatic friction effects are of comparable magnitude, so that a slight blue shift results, in agreement with well-known but puzzling experimental findings. The observed line broadening is shown to be roughly equally caused by adiabatic and non-adiabatic friction contributions for both, the stretch and bend modes in liquid water. Thus, the understanding of infrared vibrational frequencies and line shapes is considerably advanced by the quantitative analysis of the time-dependent friction that acts on vibrational modes in liquids.

==> kernelParams/dft_nvt_256_oha_kernel_fitParamsTable_G_3Exp15Osc.tex <==
$\gamma_i$ [u/ps]& $\tau_i^e$ [ps]& \\ \hline 
  4 & 9.06e-06 &  \\ 
3273 & 0.105 &  \\ 
25087 & 1.11 &  \\ 
\hline $k_i$ [u/ps$^2$] & $\tau_i^o$ [ps] & $\omega_i$ [THz]\\ \hline 
7902 & 0.0154 & 1.28e+03 \\ 
1160 & 0.0257 & 253 \\ 
2151 & 0.0277 & 413 \\ 
1380 & 0.0357 & 564 \\ 
2232 & 0.0411 & 150 \\ 
1579 & 0.0422 & 307 \\ 
1731 & 0.0484 & 595 \\ 
1606 & 0.0593 & 619 \\ 
1328 & 0.0683 & 639 \\ 
1522 & 0.0785 & 114 \\ 
1084 & 0.0812 & 658 \\ 
33879 & 0.0877 & 37 \\ 
825 & 0.103 & 674 \\ 
1110 & 0.127 & 94 \\ 
565 & 0.138 & 687 \\ 

